Open3DIS: Open-Vocabulary 3D Instance Segmentation with 2D Mask Guidance

We introduce Open3DIS, a novel solution designed to tackle the problem of Open-Vocabulary Instance Segmentation within 3D scenes. Objects within 3D environments exhibit diverse shapes, scales, and colors, making precise instance-level identification a challenging task. Recent advancements in Open-Vocabulary scene understanding have made significant strides in this area by employing class-agnostic 3D instance proposal networks for object localization and learning queryable features for each 3D mask. While these methods produce high-quality instance proposals, they struggle with identifying small-scale and geometrically ambiguous objects. The key idea of our method is a new module that aggregates 2D instance masks across frames and maps them to geometrically coherent point cloud regions as high-quality object proposals addressing the above limitations. These are then combined with 3D class-agnostic instance proposals to include a wide range of objects in the real world. To validate our approach, we conducted experiments on three prominent datasets, including ScanNet200, S3DIS, and Replica, demonstrating significant performance gains in segmenting objects with diverse categories over the state-of-the-art approaches.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
This paper addresses the challenging problem of open-vocabulary 3D point cloud instance segmentation (OV-3DIS). Given a 3D scene represented by a point cloud, we seek to obtain a set of binary instance masks of any classes of interest, which may not exist during the training phase. This problem arises to overcome the inherent constraints of the conventional fully supervised 3D instance segmentation (3DIS) approaches \cite{yi2019gspn, zhang2021point,he2021dyco3d,he2022pointinst3d,sun2022superpoint, vu2022softgroup,ngo2023isbnet, Schult23ICRA}, which are bound by a closed-set framework -- restricting recognition to a predefined set of object classes that are determined by the training datasets. This task has a wide range of applications in robotics and VR systems. This capability can empower robots or agents to identify and localize objects of any kind in a 3D environment using textual descriptions that detail names, appearances, functionalities, and more.

% \khoi{Why this is difficult/challenging?, list some applications of this problem}


% \begin{figure}[t]
%   \centering
%   \includegraphics[width=1.0\linewidth]{images/teaser2}
%    % \vspace{-4pt}
%    \caption{\textbf{Existing OV-3DIS approaches and ours.} To obtain 3D masks, OpenMask3D \cite{openmask3d} classifies class-agnostic 3D proposals using projected 2D mask features whereas OVIR-3D \cite{ovir3d} back-projects predicted 2D instance masks to 3D spaces. They have their own limitations. We propose a new approach that complements two sources of 3D proposals to overcome their limitations.}
%    \label{fig:teaser}
%    \vspace{-16pt}
% \end{figure}



% Despite remarkable attempts made in open-vocabulary 2D image understanding \cite{liang2023ovseg, xu2023open, kirillov2023segmentanything, liu2023groundingdino, zou2022xdecoder}, the OV-3DIS is still under progress due to the lack of large-scale 3D foundation models, which are the key success behind the breakthroughs in the 2D domain. 

% \cite{openscene} made a step toward 3D semantic understanding by lifting 2D image features from vision-language models such as CLIP\cite{radford2021clip}, and LSeg to 3D. Inspired by this, a line of research has emerged to address the complex task of open-vocabulary 3D point cloud instance segmentation \cite{pla,ding2023lowis3d,openmask3d,ovir3d}

There are a few studies addressing the OV-3DIS so far \cite{pla,ding2023lowis3d,openmask3d,ovir3d}. Most recently, \cite{openmask3d} proposes the use of a pre-trained 3DIS model instance proposals network to capture the geometrical structure of 3D point cloud scenes and generate high-quality instance masks. However, this approach faces challenges in recognizing rare objects due to their incomplete appearance in the 3D point cloud scene and the limited detection capabilities of pre-trained 3D models for such infrequent classes. Another approach involves leveraging 2D off-the-shelf open-vocabulary understanding models \cite{ovir3d, sam3d} to easily capture novel classes. Nevertheless, translating these 2D proposals from images to 3D point cloud scenes is a challenging task. This is because of the fact that 2D proposals capture only the visible portions of 3D objects and may also include irrelevant 
regions, such as the background. These two approaches are summarized in Fig.~\ref{fig:teaser}.

In this work, we introduce \Approach, a method for OV-3DIS that extends the understanding capability beyond predefined concept sets. Given an RGB-D sequence of images and the corresponding 3D reconstructed point cloud scene, \Approach~addresses the limitations of existing approaches. It complements two sources of 3D instance proposals by employing a 3D instance network and a 2D-Guided-3D Instance Proposal Module to achieve sufficient 3D object binary instance masks. The module (our key contribution) extracts geometrically coherent regions from the point cloud under the guidance of 2D predicted masks across multiple frames and aggregates them into higher-quality 3D proposals. 
Later, Pointwise Feature Extraction aggregates CLIP features for each instance across multiple views and in a multi-scale manner, creating instance-aware point cloud features for open-vocabulary instance segmentation.

% To evaluate the open-vocabulary capability of \Approach, we conduct evaluations on common datasets, including ScanNetV2 \cite{dai2017scannet}, S3DIS \cite{armeni20163d}, and the large-scale ScanNet200 \cite{scannet200}.
To assess the open-vocabulary capability of \Approach, we conduct experiments on the ScanNet200 \cite{scannet200}, S3DIS \cite{armeni20163d}, and Replica \cite{straub2019replica} datasets. \Approach~achieves state-of-the-art results in OV-3DIS, surpassing prior works by a significant margin. 
Especially, \Approach~delivers a noteworthy performance improvement of ${\sim}1.5$ times compared to the leading method on the large-scale dataset ScanNet200.

In summary, the contributions of our work are as follows:
\begin{enumerate}[leftmargin=7.5mm]
    % \item We propose ~\Approach, the first approach that can leverage both 3D class-agnostic proposals and 2D open-vocabulary instance masks to cover a wide range of objects in 3D environment.
    % \item We propose \Approach, an approach for open-vocabulary 3D instance segmentation, that leverages 2D-guide-3D Instance Proposal Module to generate high-quality 3D proposals.
    % with the ability to identify and segment diverse objects in a 3D scene.
    % and Pointwise Feature Extraction to obtain featured point cloud.
    
    % with the ability to identify and segment diverse objects in a 3D scene. 
    % \item The 2D-guide-3D Instance Proposal Module crafts high-quality 3D instance proposals via Agglomerative clustering by fusing 2D instance masks from 2D RGB-D images.
    % \item We propose \Approach, the first approach that exploits the strengths of both 3D class-agnostic proposals and 2D open-vocab segmentation, marking the ability to identify and segment diverse objects in a 3D world.
    % \item We introduce the Mask-guided Superpoint Grouping to generate high-quality 3D proposals from 2D instance masks from multi-view RGB-D images.
    \item We present the ``2D-Guided-3D Proposal Module'' creating precise 3D proposals by clustering cohesive point cloud regions using aggregated 2D instance masks from multi-view RGB-D images.
    \item We introduce a novel pointwise feature extraction method for open-vocabulary 3D object proposals.
    % \kalo{revise, mention bottom-up/agglomerative merging}
    \item \Approach~achieves state-of-the-art results on ScanNet200, S3DIS, and Replica datasets, exhibiting comparable performance to fully supervised methods.
\end{enumerate}

% \kalo{it is  redundant to include these summaries since the organization is pretty stadard}
%In the following, Sec.~\ref{sec:relatedwork} reviews prior work; Sec.~\ref{sec:method} specifies~\Approach; and Sec.~\ref{sec:exp} presents our experimental results. Sec.~\ref{sec:conclusion} concludes with some remarks and discussions.

% figure $->$ intro $->$ results

% proposes using a pre-trained 3DIS model to generate a set of 3D class-agnostic proposals. These proposals are then projected onto multiple viewpoints, with the top K views—determined by the highest number of projected points—being chosen for further processing. The selected images are leveraged to extract CLIP features, which are then used for classifying the 3D proposals. Nonetheless, this approach encounters difficulties in recognizing rare objects due to their incomplete appearance in the 3D point cloud scene and the limited detection capabilities of pre-trained 3D models for such infrequent categories. 
% Most recently, \cite{ovir3d} proposes using a 2D open-vocabulary detector to generate extensive 2D object proposals, then merge proposals from multiple views to obtain a set of 3D instances. However, 2D images usually capture partial views of a given 3D scene, making this method struggle to fully reconstruct the complete form of objects in the 3D space. 
% \khoi{Please rewrite, just describe the typical approach, i.e. OpenMask3D, and its limitations, don't need the whole related work here!}






% Comment of Dr Khoi
% What problem needs to be solved?


% Why is it important and why is it difficult/challenging?


% What are typical approaches for this problem and their limitations?


% How do you overcome these limitations and the motivation behind your decision?


% How do you evaluate your proposed method? (on which datasets and the important results you discover)

% Briefly summarize your contributions 

% The structure of the following sections.

% To address these limitations, 
